Towards Physically Executable 3D Gaussian for Embodied Navigation

3D Gaussian Splatting (3DGS), a 3D representation method with photorealistic real-time rendering capabilities, is regarded as an effective tool for narrowing the sim-to-real gap. However, it lacks fine-grained semantics and physical executability for Visual-Language Navigation (VLN). To address this, we propose SAGE-3D (Semantically and Physically Aligned Gaussian Environments for 3D Navigation), a new paradigm that upgrades 3DGS into an executable, semantically and physically aligned environment. It comprises two components: (1) Object-Centric Semantic Grounding, which adds object-level fine-grained annotations to 3DGS; and (2) Physics-Aware Execution Jointing, which embeds collision objects into 3DGS and constructs rich physical interfaces. We release InteriorGS, containing 1K object-annotated 3DGS indoor scene data, and introduce SAGE-Bench, the first 3DGS-based VLN benchmark with 2M VLN data. Experiments show that 3DGS scene data is more difficult to converge, while exhibiting strong generalizability, improving baseline performance by 31% on the VLN-CE Unseen task. Our data and code are available at: https://sage-3d.github.io.

==> tex/3_Method_12.1.tex <==
\begin{figure*}[!t]
\includegraphics[width=1\textwidth]{figure/Overview_9.25.pdf}
\vspace{-15pt}
\centering\caption{Overview of SAGE-3D, which consists of two key components: (1) Object‑Level Semantic Grounding, 3DGS data is annotated by expect at the object level, then be transformed into 2D semantic maps for path planning and instruction generation; (2) Physics‑Aware Execution Jointing, where scene and object collision bodies are generated via convex hull decomposition, integrated into 3DGS to form a 3DGS‑Mesh Hybrid Representation, with extensive physics simulation interfaces.}
\label{fig:model_structure}
\vspace{-17pt}
\end{figure*}



% \vspace{-12pt}
\section{SAGE-3D}
\label{sec:sage-3D}

\vspace{-10pt}

In this section, we systematically introduce \textbf{SAGE-3D}, a novel embodied learning paradigm based on 3DGS, as illustrated in Fig.~\ref{fig:model_structure}. We first provide a formal definition of this paradigm (Section~\ref{3.1}), followed by an introduction add fine-grained semantic labels to 3DGS through manual annotation and the generation of 2D top-down semantic maps (Section~\ref{3.2}). We then utilize convex hull decomposition to extract collision bodies and construct a rich physical simulation interface (Section~\ref{3.3}).



\vspace{-8pt}
\subsection{SAGE-3D Paradigm}
\label{3.1}


\vspace{-5pt}
We propose \textbf{SAGE-3D} (\textbf{S}emantically and Physically \textbf{A}ligned \textbf{G}aussian \textbf{E}nvironments for \textbf{3D} Navigation), a new paradigm that uses 3DGS as the environment foundation for training and evaluating embodied agent. This paradigm \textbf{upgrades 3DGS, originally used solely for photorealistic rendering, into an executable, semantically and physically aligned environment foundation} that supports continuous Vision-and-Language navigation and related tasks.

Formally, we define \textbf{SAGE-3D} as the process of transforming a Gaussian primitive set $G$ from a 3DGS scene, with added semantics $M$ and physics $\Phi$, into an executable environment:

\vspace{-10pt}
$$
G \;+\; M \;+\; \Phi \;\longrightarrow\; \mathcal{E}_{\mathrm{exec}}
$$
\vspace{-10pt}

where $G = \{ g_i \}_{i=1}^N$ is the set of Gaussian primitives, $M$ is the semantic layer (e.g., instance/category maps, attributes), and $\Phi$ is the physics layer (e.g., collision bodies, dynamics). The resulting environment can be formalized as a semantics- and physics-augmented POMDP (Partially Observable Markov Decision Process):

\vspace{-10pt}
$$
\mathcal{E} = (\mathcal{U}, \mathcal{S}, \mathcal{A}, \mathcal{O}, T, Z; M, \Phi),
$$
\vspace{-10pt}

where $\mathcal{U}$ is the instruction space, $\mathcal{S}$ the continuous state space, $\mathcal{A}$ the action space, $\mathcal{O}$ the multimodal observation space, and $T, Z$ are physics-driven state transition and rendering functions.

The core goal of this paradigm is to preserve the photorealistic rendering quality of 3DGS while introducing object-level semantics and physical executability, making 3DGS a viable environment foundation for training and evaluating embodied agents.




\subsection{Object‑Level Semantic Grounding}
\label{3.2}

Conventional 3DGS encodes appearance (e.g., color, density) but lacks instance IDs or object attributes, limiting precise object-level VLN instructions~\citep{chen2025survey3dgaussiansplatting, li2024instancegaussianappearancesemanticjointgaussian}. To overcome this, we release InteriorGS, a manually annotated 3DGS dataset with object-level semantics, and introduce a 2D top-down semantic map generator to support instruction generation.

% To endow 3DGS scenes with fine-grained semantics that are uniquely referable by natural language, 

\textbf{InteriorGS.} We construct InteriorGS: a dataset of 1k high-fidelity indoor 3DGS scenes (752 residential interior scenes and 248 public spaces such as concert halls, amusement parks, and gyms) with double-verified object-level annotations, including object categories, instance IDs, and bounding box information. The dataset contains over 554k object instances across 755 categories, providing a dense, semantically consistent, and broadly diverse foundation for training and evaluation.

InteriorGS's 3DGS data is sampled from our artist-created mesh scenes. To achieve reliable 3DGS reconstruction in occlusion-rich indoor environments, we render an average of 3,000 camera views per scene and use the open-source GSplat pipeline~\citep{ye2025gsplat} to estimate the 3DGS parameters. The detailed sampling process is provided in Appendix B.

% During construction, to obtain reliable 3DGS reconstructions in occlusion-rich indoor environments, we render approximately 3k camera viewpoints per scene and estimate 3DGS parameters using the open-source GSplat pipeline~\citep{ye2025gsplat} with camera poses provided by the renderer. Detailed sampling procedures are described in Appendix B.


\textbf{2D Semantic Top-Down Map Generation.} Unlike scanned mesh workflows that build NavMesh (e.g., by exhaustive scene traversal in Habitat)~\citep{song2024towards, krantz2022iterative}, 3DGS lacks inherent semantics and discrete entities, making such representations infeasible. We therefore design \textbf{a 2D semantic top-down map} by projecting annotated 3D objects from InteriorGS onto the ground plane, with doors tagged by state (open / closed / half-open) and walls marked as non-traversable. Although annotations are stored as axis-aligned 3D boxes, we refine each footprint into an irregular mask by sampling object surface points, projecting them, and taking a 2D convex hull to optimize:

$$
\mathcal{M}_k = \mathrm{Fuse}\left(\mathrm{Hull}\left\{\Pi_{\mathrm{top}}(p) \mid p \in \mathrm{Surf}(o_k)\right\}\right)
$$

where $\mathcal{M}_k$ is the 2D mask for object $o_k$, $\mathrm{Surf}(o_k)$ is the set of sampled surface points of object $o_k$, $\Pi_{\mathrm{top}}$ is the projection onto the ground plane, $\mathrm{Hull(\cdot)}$ denotes the 2D convex-hull operator, and $\mathrm{Fuse}(\cdot)$ merges multi-view masks into a consistent footprint.

% The resulting semantic top-down map $S_{top}$ contains instance IDs, category labels, functional-area tags, and coarse occupancy information, serving as the semantic layer for instruction generation.




\subsection{Physics-Aware Execution Jointing}
\label{3.3}

3DGS with semantics still cannot serve directly as a VLN environment, as it allows issues such as mesh penetration that hinder embodied learning~\citep{Yue_2024}. To overcome this, we extract object‑level collision geometry, derive navigable space, and provide a physics simulation interface.


% \textbf{Collision Body Jointing.} Each object $o_k$ from the Gaussian set is converted into a rigid-body collision shape and aligned with its semantic identifier. The conversion follows these steps: We voxelize the object's spatial support, reconstruct an isosurface from the resulting occupancy grid, and decompose the reconstructed surface mesh into convex parts to ensure stable and efficient collision detection. Formally, the collision body is denoted as
% $$
% B_k = F_{\mathrm{body}}(o_k), \quad \Phi_k = (B_k, p_k),
% $$
% where $B_k$ is the geometric collision model for object $o_k$, and $p_k$ is its physical property set including mass, friction coefficient, restitution, and inertia.


% \textbf{Physics Simulation with 3DGS–Mesh Hybrid Representation.} Starting from version 5.0, Isaac Sim supports  3DGS data into USDZ files~\citep{wu20253dgut}, which, combined with our collision bodies, enables physics simulation directly on 3DGS scenes. In Isaac Sim, each object is loaded as a USD prim and attached with $\Phi_k$ to establish rigid-body and contact properties. By default, objects in static scenes are treated as static bodies, while a small subset is set as movable or articulated to support extended interactions. Robot APIs are provided for units such as Unitree G1, Go2, and H1, with action interfaces supporting both discrete control (turn/forward) and continuous control $(v, \omega)$. Available enviroment information include RGB, depth, semantic segmentation, pose, and contact events. The environment integrates built-in collision detection, stuck/interpenetration monitoring, and recovery mechanisms, and caches offline-generated collision bodies to accelerate loading and ensure evaluation stability.

\textbf{Physics Simulation with 3DGS–Mesh Hybrid Representation.} Starting with version 5.0, Isaac Sim supports rendering 3DGS assets from USDZ files exported by 3DGUT~\citep{wu20253dgut}. However, the imported 3DGS are appearance-only and do not carry physics. To enable physically executable scenes, we take the artist-created triangle meshes of each object and apply CoACD~\citep{wei2022coacd} for convex decomposition, yielding per-object \textbf{collision bodies}. We then assemble a USDA scene where the collision bodies are authored as \emph{invisible} rigid shapes (driving contact and dynamics), while the 3DGS file remain \emph{visible} and provide photorealistic appearance. Concretely, each object is instantiated as a USD prim and augmented with $\Phi_k$ (rigid-body and contact parameters), where static-scene objects default to static bodies, and a curated subset is configured as movable or articulated to support extended interactions. This 3DGS–Mesh Hybrid Representation authoring removes the need to ray trace the artist meshes at runtime, preserves high-fidelity rendering through 3DGS, and supplies accurate collision geometry for physics.



\textbf{Agents, Control, and Observations in a Continuous Environment.} The simulator exposes robot APIs for legged and wheeled ground platforms (e.g., Unitree G1 / Go2 / H1) \emph{and} aerial robots (e.g., quadrotor UAVs). Action interfaces support both discrete commands (e.g., \texttt{turn}/\texttt{forward}/\texttt{stop}) and continuous control—velocity commands $(v,\omega)$ for ground robots and 6-DoF velocity/attitude commands for UAVs—executed in a continuous environment (metric 3D space, no teleportation between panoramic nodes). The environment provides synchronized RGB, depth, semantic segmentation, poses, and contact events, along with built-in collision detection, stuck/interpenetration monitoring, and recovery. Offline-generated collision bodies are cached to accelerate loading and ensure stable, repeatable evaluation.







\begin{figure*}[!t]
\includegraphics[width=1\textwidth]{figure/SAGE-Bench_9.25.pdf}
\vspace{-20pt}
\centering\caption{Overview of SAGE-Bench. SAGE‑Bench includes a hierarchical instruction generation scheme, two major task types, two episode complexity categories, and three newly designed natural continuity metrics for navigation.}
\label{fig:sage-bench}
\vspace{-15pt}
\end{figure*}



\section{SAGE-Bench}
\label{sec:sage-Bench}

\vspace{-10pt}

In this section, we introduce SAGE-Bench, the first 3DGS-based VLN benchmark, as shown in Fig.~\ref{fig:sage-bench}. It includes a hierarchical instruction generation scheme (Section~\ref{4.1}), a three-axis evaluation framework (Section~\ref{4.2}), and three navigation natural continuity metrics (Section~\ref{4.3}).

% as shown in Fig.~\ref{fig:sage-bench}. We begin by presenting our VLN data generation pipeline,

\vspace{-10pt}

\subsection{Data Generation}
\label{4.1}

\vspace{-5pt}

\textbf{Hierarchical Instruction Generation.} To address the limitations of current benchmarks~\citep{wang2023scalevln}, particularly the lack of tasks with causal dependencies such as ``\underline{I'm thirsty}, get water from the table'', we introduce a hierarchical scheme that combines high-level semantics with low-level action primitives for more realistic navigation.


% To address the limitations of current benchmarks~\citep{wang2023scalevln} with step-by-step instructions, we introduce a hierarchical scheme that merges high-level semantics with low-level action primitives for more realistic navigation.


We define two levels of instructions: \textbf{High-level instructions} emphasize task semantics and human-oriented intent, and comprise 5 categories: \textit{Add Object} (introducing causal objects or actions that make a trajectory contextually meaningful); \textit{Scenario Driven} (embedding specific situational motives that make the destination a reasonable place for execution); \textit{Relative Relationship} (distinguishing similar nearby targets via spatial relations such as ``next to'' or ``opposite''); \textit{Attribute-based} (identifying a unique target using perceivable attributes like color, state, or contents); \textit{Area-based} (directing the agent toward a general functional area rather than a specific object). \textbf{Low-level instructions} focus on control and kinematic evaluation, including primitive actions such as forward moves. Detailed design and explanation can be found in Appendix C.

% , and step-by-step navigation where the agent reaches a specific room or object.
% For each trajectory, we generate multiple linguistic expressions. For each high-level type, three distinct paraphrases are generated to enhance linguistic diversity.

Low-level instructions are created by templating the start and end waypoints. High-level instructions are generated by feeding an MLLM with a prompt (detailed in Appendix C) constructed from object categories, attributes, and spatial relations in the 2D semantic map.


\textbf{Trajectory Generation.} Using the collision bodies from Section~\ref{3.1}, we construct the final navigation map by combining a 1.2 m-height occupancy map with the 2D semantic map. Then we run A*-based shortest-path search to generate trajectories, more details can be found in Appendix A. 

In total, we produce 2M new instruction–trajectory pairs for VLN. We balance the data distribution and select 1,148 samples to form the SAGE‑Bench test split, including 944 high‑level and 204 low‑level samples across 35 distinct scenes, with the remainder used for training and validation.

% \textbf{Trajectory Generation.} We run A*-based shortest-path search to generate trajectories with a cost function that integrates free-space distance, narrow-passage penalties, and area preferences to ensure both obstacle avoidance and task feasibility. To diversify the dataset, start–end pairs are sampled across different rooms, functional areas, and object instances, and a minimum safety distance is enforced to avoid overly close viewpoints that would reduce the richness of the visual signal.


\vspace{-10pt}

\subsection{Three‑Axis Evaluation Framework}
\label{4.2}

\vspace{-5pt}

SAGE-Bench introduces a three-axis evaluation framework that orthogonally combines task types, instruction level, and episode complexity into discrete evaluation slices.



\textbf{Task Types.} This axis specifies the task paradigm and input form, considering two fundamental navigation tasks: VLN and No-goal Navigation (Nogoal-Nav). Nogoal-Nav aims to drive the model to explore the environment as much as possible in order to test policy understanding of the environment and the safety of exploration. We select 100 scenes as the test set for Nogoal-Nav.

% VLN takes text and images as input, provides a concrete action goal, and evaluates whether the agent correctly grounds to the target. 

\textbf{Instruction Level.} This axis measures how semantic and structural complexity affects the model, and it is aligned with the hierarchical instruction generation scheme described in Section~\ref{4.1}.

\textbf{Episode Complexity.} This axis quantifies task complexity, covering both scene complexity and path complexity. Scene complexity primarily refers to asset density: we define scenes with more than 376 assets as ``many'' and those with fewer than 184 assets as ``few''. Path complexity considers path length: we define paths longer than 29.0 m as ``long'' and those shorter than 8.4 m as ``short''.



\vspace{-10pt}

\subsection{Navigation Natural Continuity Metric}
\label{4.3}

\vspace{-5pt}

% In VLN evaluation, binary or endpoint-based metrics such as Success Rate (SR) fail to reflect the overall execution quality in a continuous, physically executable environment~\citep{li2024visionlanguagenavigationcontinuallearning}. 

As a new continuous navigation benchmark, to assess VLN model performance from the perspective of continuous motion, SAGE-Bench introduces three natural continuity metrics for navigation.

\textbf{Continuous Success Ratio (CSR).} It indicates the fraction of time the agent stays within a permissible corridor around the reference path. SR makes a 0/1 judgment only at the endpoint, whereas CSR measures the proportion of time the agent stays within a permissible corridor around the reference path while satisfying task conditions, thus reflecting ``goal‑consistent'' behavior throughout the episode. Given a trajectory of length $T$, let 
\(
s(t) = 
\begin{cases} 
1, & \mathrm{pos}(t)\in\mathcal{C} \ \text{and task conditions satisfied}\\
0, & \text{otherwise}
\end{cases}
\)
where $\mathcal{C}$ is defined by buffering the reference path with radius $r_{\text{tol}}$, then

\vspace{-10pt}
\[
\mathrm{CSR} = \frac{1}{T}\sum_{t=1}^T s(t) .
\]
\vspace{-10pt}

% CSR tolerates small spatial deviations, can be computed stage‑wise for multi‑step semantic tasks, and applies to both low‑ and high‑level goals.

\textbf{Integrated Collision Penalty (ICP).} It measures the time-averaged collision intensity along the trajectory, capturing both the frequency and duration of contacts. Traditional collision rate (CR) does not distinguish between occasional contact and persistent scraping. ICP integrates the collision intensity sequence $c(t)\in[0,1]$ over time as a penalty:

\vspace{-10pt}
\[
\mathrm{ICP} = \frac{1}{T}\sum_{t=1}^T c(t),
\]
\vspace{-10pt}

% or equivalently in continuous‑time form. A higher ICP indicates more frequent or prolonged collisions, directly reflecting physical safety during execution.

\textbf{Path Smoothness (PS).} It evaluates a normalized smoothness score derived from consecutive heading-change (or curvature) magnitudes, where higher values indicate smoother paths. Smoother paths reduce abrupt turns and acceleration changes, benefiting real robot feasibility and stable planning. PS is computed from the variance of consecutive heading changes:

\vspace{-10pt}
\[
\mathrm{PS} = 1 - \frac{1}{T-1}\sum_{t=2}^T \min\left(\frac{|\Delta \theta_t|}{\pi},1\right), \quad \Delta \theta_t = \theta_t - \theta_{t-1}, 
\]
\vspace{-10pt}

Here $\theta_t$ denotes the agent’s heading angle at trajectory time step $t$, and $\Delta \theta_t$ is the change in heading between two consecutive time steps. 

% The PS score is normalized to $[0,1]$ with larger values indicating smoother trajectories. 

% Together with CSR and ICP, it provides a multi-dimensional assessment of execution quality in continuous physical environments—an aspect absent from traditional discrete VLN benchmarks.

==> tex/4_Experiments_12.1.tex <==
\vspace{-10pt}

\section{Experiments}
\label{sec:experiments}

\vspace{-6pt}

\subsection{Experimental Setup}
\label{5.1}

\vspace{-6pt}

\textbf{Baseline.} Considering the current generalization capability of MLLM models, we conducted evaluations on a wide range of models. \textbf{(1) Closed-source MLLMs as Agent}: Includes Qwen-VL-MAX~\citep{Qwen-VL}, GPT-4.1, GPT-5. \textbf{(2) Open-source MLLMs as Agent}: Qwen2.5-VL-7B~\citep{Qwen-VL}, InternVL-2.5-8B~\citep{zhu2025internvl3}, InternVL-3-8B~\citep{chen2024expanding}, Llama-3.2-11B. \textbf{(3) Vision-Language Models}: We selected VLN models that have been widely used in recent years, including NaviLLM~\citep{zheng2024towards}, NavGPT-2~\citep{zhou2024navgpt2}, CMA~\citep{10.1007/978-3-030-58604-1_7}, NaVid~\citep{zhang2024navid}, and NaVILA~\citep{cheng2024navila}.

\textbf{Evaluation Metric.} \textbf{(1) For the VLN task.} In addition to the three novel metrics we proposed in Section~\ref{4.3} for evaluating the natural continuity of model navigation — CSR, ICP, and PS — we also adopt common metrics used in VLN tasks, including success rate (SR), oracle success rate (OSR), and success weighted by path length (SPL) and Collision Rate (CR). \textbf{(2) For the No-goalNav task.} There are two metrics: Episode Time and Explored Areas. An episode is terminated immediately if a collision occurs, and the maximum episode time is set to 120 seconds.

% To validate the effectiveness of our novel 3DGS scene data, 

\textbf{Implementation Details.} We selected 500k ``trajectory–instruction'' pairs from SAGE-Bench, with no overlap with the test set. We trained two models on this subset: one based on NaVILA's pre-trained model navila-siglip-llama3-8b-v1.5-pretrain (denoted as NaVILA-base), producing NaVILA-SAGE; and the other based on Navid's pre-trained model navid-7b-full-224 (denoted as NaVid-base), producing NaVid-SAGE. Training details are shown in Appendix A.

%  We selected 500K ``trajectory–instruction'' pairs from SAGE-Bench, with no overlap with the test set. We trained two models on this subset: one based on NaVILA's pre-trained model navila-siglip-llama3-8b-v1.5-pretrain (denoted as NaVILA-base), producing NaVILA-SAGE; and the other based on Navid's pre-trained model navid-7b-full-224 (denoted as NaVid-base), producing NaVid-SAGE. Training was carried out on 8 NVIDIA Tesla H20 GPUs with a batch size of 256 and a learning rate of $2 \times 10^{-5}$. The training data did not include any VLN-CE R2R or RxR samples.


\begin{table*}[!t]
\caption{Comparison of different models on VLN and Nogoal-Nav tasks on SAGE-Bench. \textbf{Bold} values represent the best performance across all methods.}
\vspace{-5pt}
\renewcommand{\arraystretch}{1.3} % 增加行距
\resizebox{1.00\textwidth}{!}{
\begin{tabular}{lccccccc|cc}
\toprule[1.5pt] % 顶部粗线
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{7}{c|}{\textbf{VLN (High-level Instruction)}} & \multicolumn{2}{c}{\textbf{Nogoal-Nav}} \\
& \textbf{SR} $\uparrow$ & \textbf{OSR} $\uparrow$ & \textbf{SPL} $\uparrow$ & \textbf{CR} $\downarrow$ & \textbf{CSR} $\uparrow$ & \textbf{ICP} $\downarrow$ & \textbf{PS} $\uparrow$ & \textbf{Episode Time} $\uparrow$ & \textbf{Explored Areas} $\uparrow$ \\
\midrule
\rowcolor{green!20} \multicolumn{10}{c}{\textit{Closed-source MLLMs as Agent}} \\
Qwen-VL-MAX & 0.14 & 0.25 & 0.12 & 0.85 & 0.21 & 0.41 & 0.79 & 64.74 & 6.40 \\
GPT-4.1 & 0.13 & 0.21 & 0.12 & 0.72 & 0.19 & 0.35 & 0.81 & 67.70 & 3.00 \\
GPT-5 & 0.12 & 0.18 & 0.11 & 0.63 & 0.18 & 0.24 & 0.86 & 64.60 & 2.16 \\
\midrule
\rowcolor{orange!20} \multicolumn{10}{c}{\textit{Open-source MLLMs as Agent}} \\
Qwen2.5-VL-7B & 0.13 & 0.14 & 0.13 & 0.71 & 0.21 & 0.27 & 0.87 & 42.19 & 6.88 \\
InternVL-2.5-8B & 0.10 & 0.13 & 0.10 & 0.52 & 0.14 & 0.33 & 0.88 & 28.82 & 4.28 \\
InternVL-3-8B & 0.12 & 0.20 & 0.11 & 0.64 & 0.17 & 0.32 & 0.82 & 34.70 & 6.34 \\
Llama-3.2-11B & 0.13 & 0.18 & 0.14 & 0.74 & 0.16 & 0.29 & 0.83 & 38.45 & 6.68 \\
\midrule
\rowcolor{purple!20} \multicolumn{10}{c}{\textit{Vision-Language Model}} \\
NaviLLM & 0.05 & 0.06 & 0.05 & 0.21 & 0.09 & 0.24 & 0.90 & 18.73 & 5.74 \\
NavGPT-2 & 0.10 & 0.12 & 0.11 & 0.33 & 0.14 & 0.29 & 0.83 & 24.51 & 3.36 \\
CMA & 0.13 & 0.15 & 0.14 & 0.54 & 0.26 & 0.28 & 0.86 & 44.26 & 3.22 \\
NaVid & 0.15 & 0.17 & 0.15 & 1.24 & 0.29 & 0.33 & 0.89 & 56.13 & 4.28 \\
NaVILA & 0.39 & 0.47 & 0.34 & 3.28 & 0.48 & 0.61 & 0.68 & 77.82 & 8.40 \\
\midrule
NaVid-base & 0.10 & 0.13 & 0.10 & 0.33 & 0.15 & 0.28 & 0.84 & 20.37 & 3.42 \\
\textbf{NaVid-SAGE (Ours)} & 0.36 & 0.46 & 0.32 & 2.12 & 0.48 & 0.66 & 0.54 & 60.35 & 5.66 \\
NaVILA-base & 0.21 & 0.26 & 0.22 & 1.66 & 0.33 & 0.72 & 0.41 & 58.26 & 6.52 \\
\textbf{NaVILA-SAGE (Ours)} & \textbf{0.46} & \textbf{0.55} & \textbf{0.48} & 2.67 & \textbf{0.57} & 0.54 & 0.74 & \textbf{82.48} & \textbf{8.74} \\
\bottomrule[1.5pt] % 底部粗线
\end{tabular}
}
\label{tab:result_on_sage-bench}
\vspace{-7pt}
\end{table*}




\begin{table}[!t]
\caption{Rendering speed and training convergence comparison.}
\vspace{-8pt}
\centering
\renewcommand{\arraystretch}{1.4} % 增加行间距
\resizebox{0.95\linewidth}{!}{ % 调整表格宽度以适应单栏
\begin{tabular}{lcccc}
\toprule[1.2pt]
\textbf{Environment Type} & \textbf{Avg. Render Time / Frame (ms)} $\downarrow$ & \textbf{Avg. Memory (MB)} $\downarrow$ & \textbf{Iters to SR=40\% (k)} $\downarrow$ & \textbf{Time-to-SR=40\% (hrs)} $\downarrow$ \\
\midrule
Scanned Mesh (MP3D/HM3D) & 16.7 & 850 & 120 & 4.8 \\
3DGS–Mesh
Hybrid Representation (Ours) & 6.2 & 220 & 160 & 6.2 \\
\bottomrule[1.2pt]
\end{tabular}
}
\label{tab:rendering_memory_training_performance}
\vspace{-7pt}
\end{table}


\begin{figure*}[!t]
\includegraphics[width=0.9\textwidth]{figure/Visualization_9.25_v2.pdf}
\vspace{-8pt}
\centering\caption{Visualization case study of navigation natural continuity. The red trajectory is the ground truth, and the blue Trajectory is the trajectory of NaVILA.}
\label{fig:visualization_study}
\vspace{-18pt}
\end{figure*}



\vspace{-3pt}

\subsection{Results and Insights}
\label{5.2}

\vspace{-3pt}




\begin{table*}[!t]
    \begin{minipage}{0.365\textwidth}
        \centering
        \caption{Results on VLN-CE.}
        \vspace{-6pt}
        \renewcommand{\arraystretch}{1.3} % 增加行距
        \resizebox{\linewidth}{!}{
        \begin{tabular}{l|ccc}
        \toprule[1.5pt] % 顶部粗线
        \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{R2R Val-Unseen}} \\
        \cline{2-4}
        & \textbf{SR} $\uparrow$ & \textbf{OSR} $\uparrow$ & \textbf{SPL} $\uparrow$ \\
        \midrule
        Seq2Seq & 0.25 & 0.37 & 0.22 \\
        Navid-base & 0.22 & 0.32 & 0.17 \\
        \textbf{Navid-SAGE (Ours)} & 0.31 & 0.42 & 0.29 \\
        CMA & 0.32 & 0.40 & 0.30 \\
        NaVid & 0.37 & 0.49 & 0.36 \\
        NaVILA-base & 0.29 & 0.38 & 0.27 \\
        \textbf{NaVILA-SAGE (Ours)} & 0.38 & 0.51 & 0.36 \\
        NaVILA & 0.50 & 0.58 & 0.45 \\
        \bottomrule[1.5pt] % 底部粗线
        \end{tabular}
        }
        \label{tab:results_on_vln-ce}
    \end{minipage}
    \hfill
    \begin{minipage}{0.62\textwidth}
        \centering
        \caption{Results on different instruction levels.}
        \vspace{-6pt}
        \renewcommand{\arraystretch}{1.3} % 增加行距
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|cccccc}
        \toprule[1.5pt] % 顶部粗线
        \multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\textbf{Instruction Level}} & \multicolumn{6}{c}{\textbf{SAGE-Bench VLN}} \\
        \cline{3-8}
        & & \textbf{SR} $\uparrow$ & \textbf{OSR} $\uparrow$ & \textbf{SPL} $\uparrow$ & \textbf{CSR} $\uparrow$ & \textbf{ICP} $\downarrow$ & \textbf{PS} $\uparrow$ \\
        \midrule
        \multirow{2}{*}{\textbf{GPT-4.1}} & Low-level & 0.22 & 0.37 & 0.19 & 0.27 & 0.60  & 0.70 \\
        & High-level & 0.13 & 0.21 & 0.12 & 0.19 & 0.35 & 0.81 \\
        \multirow{2}{*}{\textbf{InternVL-3-8B}} & Low-level  & 0.20 & 0.35 & 0.18 & 0.26 & 0.61 & 0.69 \\
        & High-level & 0.12 & 0.20 & 0.11 & 0.17 & 0.32 & 0.82 \\
        \multirow{2}{*}{\textbf{NaVid}} & Low-level  & 0.24 & 0.42 & 0.21 & 0.34 & 0.63 & 0.64 \\
        & High-level & 0.15 & 0.17 & 0.15 & 0.29 & 0.33 & 0.89  \\
        \multirow{2}{*}{\textbf{NaVILA}} & Low-level  & 0.56 & 0.66 & 0.50 & 0.58 & 0.48 & 0.75 \\
        & High-level & 0.39 & 0.47 & 0.34 & 0.48 & 0.61 & 0.68 \\
        \bottomrule[1.5pt] % 底部粗线
        \end{tabular}
        }
        \label{tab:high-level_and_low-level}
    \end{minipage}%
\vspace{-10pt}
\end{table*}



\begin{figure*}[!t]
    \begin{minipage}{0.55\textwidth}
        \centering
        \captionsetup{type=table} % 告诉 LaTeX这是一个table的caption
        % \vspace{-3pt}
        \caption{Impact of the number of scenes and samples on model performance.}
        \vspace{-6pt}
        \renewcommand{\arraystretch}{1.3} % 增加行距
        \resizebox{\linewidth}{!}{
        \begin{tabular}{cc|cccccc}
        \toprule[1.5pt] % 顶部粗线
        \multicolumn{2}{c|}{Data in \# Train} & \multicolumn{6}{c}{\textbf{SAGE-Bench VLN}} \\
        \cline{3-8}
        \#Scenes & \#Samples & \textbf{SR} $\uparrow$ & \textbf{OSR} $\uparrow$ & \textbf{SPL} $\uparrow$ & \textbf{CSR} $\uparrow$ & \textbf{ICP} $\downarrow$ & \textbf{PS} $\uparrow$ \\
        \midrule
        % 800 & 480k & 0.44 & 0.51 & 0.45 & 0.54 & 0.59 & 0.66 \\
        800 & 240k & 0.42 & 0.47 & 0.42 & 0.50 & 0.61 & 0.63 \\
        800 & 120k & 0.40 & 0.43 & 0.40 & 0.48 & 0.62 & 0.62 \\
        800 & 60k  & 0.36 & 0.42 & 0.38 & 0.46 & 0.64 & 0.58 \\
        400 & 120k & 0.34 & 0.39 & 0.35 & 0.44 & 0.67 & 0.54 \\
        400 & 60k  & 0.31 & 0.37 & 0.33 & 0.43 & 0.67 & 0.52 \\
        400 & 30k  & 0.28 & 0.35 & 0.31 & 0.43 & 0.69 & 0.49 \\
        400 & 15k  & 0.25 & 0.31 & 0.27 & 0.39 & 0.70 & 0.46 \\
        200 & 60k  & 0.27 & 0.33 & 0.29 & 0.41 & 0.70 & 0.47 \\
        100 & 60k  & 0.23 & 0.29 & 0.26 & 0.38 & 0.71 & 0.44 \\
        % 800 & 240k & 0.42 & 0.47 & 0.42 & 0.50 & 0.61 & 0.63 \\
        % 800 & 120k & 0.40 & 0.43 & 0.40 & 0.48 & 0.62 & 0.62 \\
        % 800 & 60k  & 0.36 & 0.42 & 0.38 & 0.46 & 0.64 & 0.58 \\
        % 400 & 120k & 0.34 & 0.39 & 0.35 & 0.44 & 0.67 & 0.54 \\
        % 400 & 60k  & 0.31 & 0.37 & 0.33 & 0.43 & 0.67 & 0.52 \\
        % 200 & 60k  & 0.27 & 0.33 & 0.29 & 0.41 & 0.70 & 0.47 \\
        % 100 & 60k  & 0.23 & 0.29 & 0.26 & 0.38 & 0.71 & 0.44 \\
        \midrule
        \multicolumn{2}{c|}{NaVILA-base} & 0.21 & 0.26 & 0.22 & 0.36 & 0.72 & 0.41 \\
        \bottomrule[1.5pt] % 底部粗线
        \end{tabular}
        }
        \label{tab:effect_of_scenes_and_samples}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.43\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/effect_of_scenes_and_samples.png}
        \vspace{-20pt}
        \caption{Model performance change curve (number of scenes vs. sample size).}
        \label{fig:effect_of_scenes_and_samples}
    \end{minipage}
\vspace{-15pt}
\end{figure*}




\textbf{Overall Comparison on SAGE-Bench.} Tab.~\ref{tab:result_on_sage-bench} presents the experimental results of MLLMs and VLN models on SAGE-Bench. \textbf{(1) SAGE-Bench poses a novel and challenging VLN task for current VLN models and MLLMs.} Except for the recent SOTA VLN model NaVILA, other models achieve SR values no higher than 0.15. For instance, NaVid, which achieves 0.37 SR and 0.49 OSR on VLN-CE R2R Val-Unseen, only obtains 0.15 SR and 0.17 OSR on SAGE-Bench. Similarly, NaVILA, which achieves 0.54 SR and 0.63 OSR on VLN-CE R2R Val-Unseen, records only 0.39 SR and 0.47 OSR on SAGE-Bench. \textbf{(2) MLLMs' multimodal understanding inherently gives them some VLN capability.} Both the latest open-source and closed-source MLLMs achieve VLN SRs ranging from 0.10 to 0.14 on SAGE-Bench, comparable to dedicated VLN models such as CMA (0.13 SR) and NaVid (0.15 SR), and even surpass VLN models in OSR. For example, the 0.20 OSR achieved by InternVL-3 exceeds that of NaVid (0.17 OSR).


\textbf{Insight 1: 3DGS scene data renders faster than scanned mesh data but is harder to converge.} We randomly selected 10k training samples and 1k validation samples from both traditional scanned mesh data and our 3DGS data, and conducted experiments with the NaVILA-base model on an NVIDIA H20 GPU. Tab.~\ref{tab:rendering_memory_training_performance} compares the rendering speed and model convergence between scanned mesh VLN data and our 3DGS VLN data. The results show that 3DGS scene data achieves a per-frame rendering time of 6.2 ms and an average memory usage of 220 MB, outperforming the 16.7 ms and 850 MB of scanned mesh data. However, in training, to reach the same 40\% SR, the 3DGS-based model required about 160 iterations and 6.2 hours, while the scanned mesh-based model needed only about 120 iterations and 4.8 hours. This indicates that although 3DGS scene data offers faster rendering, it presents greater training difficulty and is relatively harder to converge.


\textbf{Insight 2: 3DGS scene data exhibits strong generalizability.} To evaluate the effectiveness of our novel 3DGS-based scene data, we tested the NaVILA-SAGE and NaVid-SAGE models, which were trained solely on our SAGE-Bench dataset, on the VLN-CE benchmark. As shown in Tab.~\ref{tab:results_on_vln-ce}, models trained entirely on SAGE-Bench data (without any VLN-CE data) achieved clear performance improvements over their respective baselines. For example, NaVILA-SAGE achieved a 31\% relative SR improvement on R2R Val-Unseen (from 0.29 to 0.38) and a 34\% relative OSR improvement (from 0.38 to 0.51), with similar gains observed for the NaVid model.



\textbf{Insight 3: Our newly proposed three continuity metrics enable effective study of navigation’s natural continuity, filling key gaps left by conventional metrics.} In Tab.~\ref{tab:result_on_sage-bench}, we report results for our three navigation natural continuity metrics. We observe that CSR is generally higher than SR, indicating a more inclusive and robust metric that does not require the model to fit the ground-truth trajectory exactly. For ICP and PS, although NaVILA attains relatively high task completion (0.39 SR, 0.47 OSR), it lacks natural motion continuity: an ICP of 0.61 indicates sustained collisions during navigation, and a PS of 0.68 reflects large, mechanical turning angles rather than smooth, natural motion. Additional visual examples in Fig.~\ref{fig:visualization_study} corroborate this finding: the NaVILA model (blue trajectory) exhibits unsmooth movement and persistent collisions that conventional metrics fail to reveal. For instance, in Case 1, the model hugs the wall for a long period, yet the collision rate CR is only 1, while our ICP reaches 0.87. 

% These results demonstrate that our approach makes 3DGS a viable environment for continuous navigation.









\vspace{-6pt}

\subsection{More Findings}
\label{5.4}

\vspace{-5pt}

\textbf{High-level Instructions vs. Low-level Instructions.} Tab.~\ref{tab:high-level_and_low-level} compares the performance of different models on high-level and low-level instructions in the VLN task.Compared with low‑level instruction data, which are composed of basic step‑by‑step actions that guide the model gradually through the task, VLN models perform worse when executing high‑level instructions. Even the recent SOTA model NaVILA achieves only a 0.39 success rate on high-level instructions, significantly lower than its 0.56 success rate on low-level instructions. Notably, high-level instructions, with their more natural semantics, are closer to real-life scenarios, presenting greater challenges for the future development of VLN models.

\textbf{Number of training Scenes vs. Training Sample Size.} Tab.~\ref{tab:effect_of_scenes_and_samples} and Fig.~\ref{fig:effect_of_scenes_and_samples} illustrate the influence of varying the number of scenes and the number of samples. We observe that increasing the number of scenes in the training data, while keeping the sample size constant, yields greater performance gains than merely increasing the number of samples. Specifically, with the same number of augmented scenes (800), increasing the sampling density progressively improves the VLN model's performance on the val-unseen split. Conversely, generating the same number of samples (700k) from a larger number of environments produces better results. These findings indicate that the number of scenes (Scenes) has a greater impact than the number of samples (Samples), suggesting that diversity of environments is more critical for learning VLN.




\begin{figure*}[!t]
\includegraphics[width=1\textwidth]{figure/three_bar_charts.png}
\vspace{-20pt}
\centering\caption{Results under Different Evaluation Slice.}
\label{fig:Results_under_Different_Evaluation_Slice}
\vspace{-15pt}
\end{figure*}



\textbf{Results under Different Evaluation Slice.} Based on our three‑axis evaluation framework, we further present experimental results in Fig.~\ref{fig:Results_under_Different_Evaluation_Slice} for different high‑level instruction types, trajectory lengths, and scene complexities. The results show that VLN models perform worse on the ``Relative Relationship'' and “Attribute‑based” instruction types, with SR scores for both NaVILA and NaVid more than 2\% lower than those for other types. In addition, as trajectory length increases and scene complexity grows, model performance drops significantly.
